Extreme clicking for efficient object annotation

Manually annotating object bounding boxes is central to building computer vision datasets, and it is very time consuming (annotating ILSVRC [53] took 35s for one high-quality box [62]). It involves clicking on imaginary corners of a tight box around the object. This is difficult as these corners are often outside the actual object and several adjustments are required to obtain a tight box. We propose extreme clicking instead: we ask the annotator to click on four physical points on the object: the top, bottom, left- and right-most points. This task is more natural and these points are easy to find. We crowd-source extreme point annotations for PASCAL VOC 2007 and 2012 and show that (1) annotation time is only 7s per box, 5x faster than the traditional way of drawing boxes [62]; (2) the quality of the boxes is as good as the original ground-truth drawn the traditional way; (3) detectors trained on our annotations are as accurate as those trained on the original ground-truth. Moreover, our extreme clicking strategy not only yields box coordinates, but also four accurate boundary points. We show (4) how to incorporate them into GrabCut to obtain more accurate segmentations than those delivered when initializing it from bounding boxes; (5) semantic segmentations models trained on these segmentations outperform those trained on segmentations derived from bounding boxes.

==> secResultsObjDet.tex <==
\section{Results on object detection}
\label{sec:resultsDet}

To further validate our scheme for annotating bounding-boxes, we present experiments on training object class detectors from them, and compare to training from boxes manually drawn used the standard scheme \vitto{pascal-voc-g}, and to alternative ways to efficiently train detectors~\cite{wsol,verification}.

%\begin{table*}[t]
%\centering
%\footnotesize
%\caption{\small \todo{Object detection results on PASCAL VOC 2007 and 2012.} \dimpp{Do we need here the quality of training bounding-boxes? It's repetition from sec 3...} }
%\scalebox{1}{
%\begin{tabular}{|c|c||c|c|c|c||c|c||c|} \hline
% &  & \multicolumn{4}{|c||}{Annotations quality} & \multicolumn{2}{|c||}{Detector performance (mAP)} & Annotation time \\ 
% \hline
%Dataset & Annotation approach & mIoU & CorLoc@90 & CorLoc@70 & CorLoc@50 & AlexNet & VGG16 & in hours \\
%\hline
%& Extreme clicks & 87.9 & 62.5 & 93.5 & 97.1 & 56.0 & 66.1 & 14.3\\
%PASCAL & PASCAL ground-truth & 100 & 100 & 100 & 100 & 55.5 & 65.9 & 70.0\\
%VOC & State-of-the-art WSOL~\cite{bilen16cvpr} & -- & -- & -- & 54.2 & 34.5 & 34.8 & 0\\
%2007 & Human verification~\cite{papadopoulos16cvpr} & 61.1 & 5.1 & 36.4 & 80.7 & 49.6 & 57.9 & 9.2\\
%& Best window proposal~\cite{dollar14eccv} & 81.6 & 17.3 & 91.0 & 98.9 & 54.1 & 65.4 & --\\
%\hline \hline
%PASCAL & Extreme clicks & 87.4 & 61.4 & 91.1 & 96.5 & 51.7 & 61.7 & 16.8\\
%VOC & PASCAL ground-truth & 100 & 100 & 100 & 100 & 51.9 & 61.7 & 79.8\\
%2012 & Best window proposal~\cite{dollar14eccv} & 81.3 & 18.7 & 89.6 & 97.7 & 50.4 & XX & --\\
%\hline
%\end{tabular}
%}
%\label{tab:objDetMAP}
%\end{table*}

\begin{table}[t]
\centering
\footnotesize
\caption{\small \todo{Object detection results on PASCAL VOC 2007 and 2012.} }
\scalebox{0.83}{
\begin{tabular}{|c|c||c|c||c|} \hline 
% &  & \multicolumn{2}{|c|}mAP} & Annotation time \\
& & \multicolumn{2}{|c|}{mAP} & Annotation time \\
 \hline
Dataset & Annotation approach & AlexNet & VGG16 & in hours \\
\hline
 & Extreme clicks & 56.0 & 66.1 & 14.3\\
PASCAL & PASCAL ground-truth & 55.5 & 65.9 & 70.0\\
VOC & State-of-the-art WSOL~\cite{bilen16cvpr} & 34.5 & 34.8 & 0\\
2007 & Human verification~\cite{papadopoulos16cvpr} & 49.6 & 57.9 & 9.2\\
& Best window proposal~\cite{dollar14eccv} & 54.1 & 65.4 & --\\
\hline \hline
PASCAL & Extreme clicks & 51.7 & 61.7 & 16.8\\
VOC & PASCAL ground-truth & 51.9 & 61.7 & 79.8\\
2012 & Best window proposal~\cite{dollar14eccv} & 50.4 & XX & --\\
\hline
\end{tabular}
}
\label{tab:objDetMAP}
\end{table}


\subsection{PASCAL VOC 2007}
\label{sec:resultsDet07}

\mypar{Dataset.}
We perform experiments on PASCAL VOC 2007~\cite{everingham10ijcv}, which consists of 20 classes across 5,011 training images (trainval) and 4,952 test images. To ensure a fair comparison we use exactly one bounding-box per class per trainval image (7,306 boxes in total) for each alternative annotation approach to train object detectors and measure their performance on the test set. \dimpp{ninja move}
\vitto{does not work as you did not say yet what we compare against; think of the right order of this section}


\mypar{Object detection model.}
As object detector we use Fast R-CNN~\cite{girshick15iccv} with EdgeBoxes~\cite{dollar14eccv} as object proposals. We use both AlexNet~\cite{krizhevsky12nips} and VGG16~\cite{simonyan15iclr} as underlying CNN architectures.

\mypar{Evaluation.}
We quantify the quality of bounding boxes on the training set with mIoU (mean intersection-over-union) and Correct Localization (CorLoc@N). \vitto{terrible writing, just copied from a completely different situation (MIL)!! Wording in 3.3 much better for this situation; @Dim: it's not always good to copy text from previous papers; only when it makes sense!! Think about the meaning of your work, and write accordingly} The latter is the percentage of images in which the bounding-box correctly localizes (with IoU $\geq N\%$) an object of the target class.  \vitto{hum ... this does not belong here but in sec. 3.3 instead; generally: FUSE THE MATERIAL IN THIS SECT 5 WITH 3.3, EITHER PUT IT ALL IN 3.3 OR ALL HERE}
%
We measure the performance of the trained object detector on the test set using mean average precision (mAP).

We measure the performance of the trained object detector on the test set using mean average precision (mAP). To ensure a fair comparison we use exactly one bounding-box per class per trainval image (7,306 boxes in total) for each alternative annotation approach to train object detectors and measure their performance on the test set. \dimpp{ninja move}
\vitto{does not work as you did not say what we compare against}

\mypar{Annotation time.}
We quantify annotation effort using actual human time measurements. For our extreme click annotations we use the total response time of our crowdsourcing framework in AMT (7.0s per box for VOC 2007) \vitto{already said in 3.3; MUST FUSE}. For PASCAL ground-truth bounding-boxes we use the annotation times for ILSVRC reported by~\cite{su12aaai}: 34.5s for drawing a single bounding-box and checking its quality \vitto{@Jasper: as we agreed, expand this better here}. These timings are representative for PASCAL VOC, since the ILSVRC images are of comparable difficulty and quality~\cite{russakovsky15ijcv}.
We compare to a weakly-supervised object localization approach, for which the effort for drawing bounding-boxes is zero. Furthermore, we compare to the human verification scheme~\cite{papadopoulos16cvpr}, using the times they report.
%=======
%\vitto{VITTO HERE}
%We quantify the annotation effort of our method compared to other methods using actual human time measurements. For our extreme click annotations we use the total response time of our crowdsourcing framework in AMT (7.0s per box for VOC 2007). For PASCAL ground-truth bounding-boxes we use the annotation times for ILSVRC reported by~\cite{su12aaai}: 34.5s for drawing a single bounding-box and checking its quality. These timings are representative for PASCAL VOC, since the ILSVRC images are of comparable difficulty and quality~\cite{russakovsky15ijcv}. We compare to a weakly-supervised object localization approach, for which the effort for drawing bounding-boxes is zero. Furthermore, we compare to the human verification in the loop scheme of~\cite{papadopoulos16cvpr}, using the times they report.
%>>>>>>> .r14406

\mypar{PASCAL ground-truth bounding-boxes~\cite{pascal-right-year}.}
Training object detectors from 7,306 \vitto{why this number? Say once clearly we do one box per image per class and that's it, applies to all methods} PASCAL ground-truth bounding-boxes results in 55.5\% mAP using AlexNet and 65.9\% mAP using the deeper VGG16 architecture. Annotating these boxes requires 70 hours of total annotation time (\vitto{do not repeat} at 34.5s per box).

\mypar{Extreme click annotations.}
The object detectors trained from bounding boxes derived from our extreme click annotation yield 56.0\% (AlexNet) and 66.1\% (VGG16) mAP. Interestingly, these detectors match the performance of those trained on the original, manually drawn ground-truth boxes. This confirms the quality of the boxes produced by our annotation scheme is as good as the original ground truth. Importantly, our scheme requires only 14.6 hours of annotation ($5\times$ less).
%=======
%The object detectors trained from bounding-boxed derived from our extreme click annotation yield 56.0\% (AlexNet) and 66.1\% (VGG16) mAP. Interestingly, these detectors match exactly the performance of those trained on the same amount of ground-truth PASCAL boxes from the exactly same images.\frank{Not so surprising, given that we achieve almost perfect overlap with the Pascal GT boxes (87.9).} More importantly, our annotation scheme requires only 14.3 hours, a speed-up in annotation time by a factor of five.
%>>>>>>> .r14406

\mypar{Weakly-supervised object localization~\cite{bilen16cvpr}.}
As a reference, we report here the mAP performance of Bilen et al.~\cite{bilen16cvpr}, a state-of-the-art WSOL technique on PASCAL VOC 2007 \vitto{why again say on PASCAL VOC 07? I thought all of this is on VOC07? It's the name of the subsection!}. WSOL techniques are very cheap in terms of annotation time but their mAP performance (34.8\% with VGG16) is just over half of what we achieve with a detector trained on extreme clicks.

\mypar{Human verification scheme~\cite{papadopoulos16cvpr}.}
This approach only requires annotators to iterative verify bounding boxes generated automatically by WSOL. This system is very efficient and requires only 9.2 hours of annotation time. However, the object detection performance is $-6.4\%$ and $-8.2\%$ below that delivered by our annotation scheme, while saving only five hours of annotation time. \dimpp{comment for the training bbs?}
\vitto{unconvincing! Focus on BBs produced at training time: from their paper you can claim a certain CorLoc @ IoU$>$0.5; we ROCK on that measure! Then as corroborating evidence you can state they reach only about 90\% of the mAP of training from gt bbs}

\mypar{Oracle best window proposals.}
\vitto{fuse with sec. 3.3}
We also train object detectors on the oracle best EdgeBox window proposal~\cite{dollar14eccv}. This yields 54.0\% mAP using AlexNet and 65.4\% mAP using VGG16. These mAPs can be seen as an upper-bound for any learning algorithm based on selecting object proposals. This includes most WSOL~\cite{cite a lot, bilen16cvpr} and the human verification scheme~\cite{papadopoulos16cvpr}.
The object detectors trained on our extreme clicks go even slightly beyond this upper-bound ($+1\%$ mAP \vitto{pending result on VOC12}).


\subsection{PASCAL VOC 2012}
\label{sec:resultsDet12}

\vitto{same story again, same conclusions! Fuse these two subsections; when stating results, say you focus on VOC07 numbers, and that the same conclusions hold on VOC12}

\mypar{Dataset and settings.}
We also perform experiments on PASCAL VOC 2012~\cite{everingham10ijcv}. We use the training set to train object detectors (5,717 images, 8,331 bounding-boxes) and test them on the validation set (5,823 images). %
We use exactly the same evaluation setup as for PASCAL VOC 2007, as described in sec.~\ref{sec:resultsDet07}.

\mypar{PASCAL ground-truth bounding-boxes.}
Training object detectors from 8,331 PASCAL ground-truth bounding-boxes that require 79.8 hours of total annotation time (at 34.5s per box) yields 51.9\% mAP (AlexNet) and 61.7\% mAP (VGG16).

\mypar{Extreme click annotations.}
Similar to PASCAL VOC 2007 above, the object detectors trained from our extreme click annotations yield the same mAP performance (51.7\% and 61.7\%) as the ones trained on PASCAL ground-truth boxes. The total annotation time needed here to collect the extreme clicks was 16.8 hours, which is again a reduction by a factor $5\times$.

\mypar{Oracle best window proposals.}
Training detectors from the oracle best EdgeBox window proposal~\cite{dollar14eccv} yields 50.4\% and XX\% mAP , again 1-2\% below those trained on our extreme click annotations.


==> secResultsObjDetFused.tex <==
\section{Experiments on extreme annotations}
\label{sec:resultsDet}

\begin{table*}[t]
\centering
\small
\caption{\small \todo{Object detection results on PASCAL VOC 2007 and 2012.} \dimpp{Do we need here the quality f training bounding-boxes? It's repetition from sec 3...} }
\scalebox{0.98}{
\begin{tabular}{|c|c||c|c|c|c||c|c||c|} \hline
 &  & \multicolumn{4}{|c||}{Annotations quality} & \multicolumn{2}{|c||}{Detector performance (mAP)} & Annotation time \\ 
 \hline
Dataset & Annotation approach & mIoU & IoU$>$0.9 & IoU$>$0.7 & IoU$>$0.5 & AlexNet & VGG16 & in hours \\
\hline
& Human agreement & 87.9 & 57.7 & 92.7 & 98.1 & -- & -- & -- \\
\hline
& Extreme clicks & 87.9 & 62.5 & 93.5 & 97.1 & 56.0 & 66.1 & 14.3\\
PASCAL & PASCAL ground-truth & 100 & 100 & 100 & 100 & 55.5 & 65.9 & 70.0\\
VOC & Best window proposal~\cite{dollar14eccv} & 81.6 & 17.3 & 91.0 & 98.9 & 54.1 & 65.4 & --\\
2007 & State-of-the-art WSOL~\cite{bilen16cvpr} & -- & -- & -- & 54.2 & 34.5 & 34.8 & 0\\
% & Human verification~\cite{papadopoulos16cvpr} & 61.1 & 5.1 & 36.4 & 80.7 & 49.6 & 57.9 & 9.2\\
& Human verification~\cite{papadopoulos16cvpr} & -- & -- & -- & 80.7 & 49.6 & 57.9 & 9.2\\
\hline \hline
PASCAL & Extreme clicks & 87.4 & 61.4 & 91.1 & 96.5 & 51.7 & 61.7 & 16.8\\
VOC & PASCAL ground-truth & 100 & 100 & 100 & 100 & 51.9 & 61.7 & 79.8\\
2012 & Best window proposal~\cite{dollar14eccv} & 81.3 & 18.7 & 89.6 & 97.7 & 50.4 & XX & --\\
\hline
\end{tabular}
}
\label{tab:objDetMAP}
\end{table*}

\subsection{Data collection}
We implemented our annotation scheme on Amazon Mechanical Turk (AMT) and we collected extreme click annotations for the trainval set of PASCAL VOC 2007~\cite{pascal07:thomas} (5011 images) and for the training set of PASCAL VOC 2012~\cite{pascal-voc-2012} (5717 images), which consist of 20 classes. Each image was annotated with four extreme clicks on one object by one single annotator for each class present in the image.
%
In our experiments we annotate a single instance per class per image resulting in 7,306 instances for PASCAL VOC 2007 and 8,331 instances for PASCAL VOC 2012. To ensure a fair comparison for each alternative annotation approach we always use exactly the same number of instances.

\vitto{not sure where to put the following ... perhaps in the experiments; now we said here that we do one object per image; the only re maining info is that other works do this too; belongs more to results, or nowhere; we do not need to apologize! We state what we do and that's it}
\dimpp{previous: In our experiments we annotate a single instance per image, as is common when using weakly supervised methods or methods which semi-automatically obtain annotations~\cite{needCitations}.}

\mypar{Annotation time.}
During the annotation stage of our crowd-sourcing framework, we measure the annotator's response time from the moment the image appears until they click for the fourth time. On PASCAL VOC 2007, the mean response time was $7.0$s leading to a total annotation time of 14.3 hours.
% with a median time of $5.3$s. 
On PASCAL VOC 2012, the mean response time was $7.2$s, leading to a total annotation time of 16.8 hours of total annotation time.
% with a median of $5.4$s. \vitto{I propose to kill the medians; the simple the story, the better? Or maybe we use the medians later somewhere?} \dimpp{No. I don't use the median, BUT for Su et al. we always use the medians...}  

We also examine the mean response time per click for PASCAL VOC 2007. Interestingly, the first click on an object takes about 2.5s, and after that the other clicks take about 1.5s. This is because of visual search: the annotator needs to find the object in the image before they can make the first click. \vitto{can we cite some cogsci paper that states 1s per image to do visual search? It would be awesome to state our observations are consistent with the findings of XYZ} \dimpp{maybe our eye-tracking paper?}

For PASCAL ground-truth bounding-boxes we use the annotation times for ILSVRC reported by~\cite{su12aaai}: 34.5s for drawing a single bounding-box and checking its quality \vitto{@Jasper: as we agreed, expand this better here}. These timings are representative for PASCAL VOC, since the ILSVRC images are of comparable difficulty and quality~\cite{russakovsky15ijcv}. So, annotating the trainval set of PASCAL VOC 2007 requires a total annotation time of 70 hours, while annotating the training set of PASCAL VOC 2012 requires 79.8 hours.
%
We also compare to a weakly-supervised object localization approach, for which the effort for drawing bounding-boxes is zero. Furthermore, we compare to the human verification scheme~\cite{papadopoulos16cvpr}, using the times they report.

\mypar{Cost.}
We paid the annotators $\$0.15$ to annotate a batch of 10 images. Based on their mean response time of 7s, this results in a wage of about $\$7.7$ per hour. The total cost for annotating the whole trainval set of PASCAL VOC 2007 and the training set of PASCAL VOC 2012 was $\$121.8$ and $\$138.9$, respectively. \dimpp{this is without the extra fees to Mturk!} \vitto{what's that?} \dimpp{on top of this 0.15\$ per batch to the annotators we have to pay some extra fees to Amazon. (that's how they make money :)). It was extra 24.66 for VOC07 and 27.99 for VOC12} 

\subsection{Quality of annotations}

We evaluate here the quality of the extreme click annotations we collected.
We first derive a bounding-box from the four clicks (each click provides one coordinate) \dimpp{In practice it's -/+ 1 pixel as the bb should contain the clicks}. Then we evaluate the intersection-over-union (IoU) with respect to the PASCAL ground-truth bounding boxes. We measure the percentage of bounding boxes we annotated per class with IoU greater than 0.5/0.7/0.9 and we report the mean over all object classes. In addition, we also report the mean IoU over all object classes (mIoU).
\vitto{confusing: so: the $>$ experiments are just percentages over the whole dataset, without taking into account that some classes have more samples; but then when you do mIoU you do it first mean within each class, and then mean over classes? That's different in two ways from the other data; why?}
\dimpp{is it ok now? should I change the IoU$>$ to mIoU$>$?}

\mypar{Human agreement}
First, we want to obtain an upper bound of quality by looking at the human agreement between expert annotators. This is possible using only PASCAL ground-truth data, since some of the images (422 trainval images for VOC 2007) have both bounding boxes and segmentation masks, annotated by different annotators. %\jasper{Dim, we have to be a bit careful here. If I remember correctly, there are no instances. So if there are multiple objects within an image, we may measure the wrong thing.}
%\dimpp{There is instance annotation on VOCseg! I always verify 1 instance per class per image where we have a bounding-box and a segmentation mask!}
Hence we can fit tight bounding boxes on the segmentation masks to generate a second set of ground-truth boxes.
This enables to measure the agreement among the expert annotators that created PASCAL. We find this agreement to be 87.9 mIoU for VOC 2007. \dimpp{I haven't done it for VOC12. should I?}

\mypar{Extreme click annotations}
Measuring the quality of our extreme click annotations \vitto{wrt to which set of gt boxes?}\dimpp{the PASCAL gt boxes...we say it exactly in the intro of this subsection.}, we find 87.9\% mIoU for VOC 2007 and 86.8\% mIoU for VOC 2012 (Table~\ref{tab:objDetMAP}). This indicates that boxes derived from our extreme click annotations are extremely accurate and in fact match the inter-annotator agreement of human experts manually drawing bounding-boxes. Moreover, ours boxes match human agreement also on the other metrics considered (i.e. IoU greater than 0.5/0.7/0.9).

\mypar{Oracle best window proposals~\cite{dollar14eccv}}
To put these results in perspective, we also compute the accuracy of the best available object proposal (among 2000 proposals per image) from Edge Boxes~\cite{dollar14eccv}. Our bounding boxes are much more accurate even compared to this oracle best proposal in terms of mIoU. We also outperform them by more than 40\% at very strict overlap values (IoU$>$0.9).

\mypar{Human verification~\cite{papadopoulos16cvpr}}
This approach only requires annotators to iteratively verify bounding boxes generated automatically by WSOL. This system is very efficient and requires only 9.2 hours of annotation time. However, the quality of the bounding-boxes they produce at training time is only 80.7\% at IoU$>$0.5. This is $-16.4\%$ below our nearly perfect 97.1\%, while saving only five hours of annotation time. 

\mypar{Influence of qualification test and quality control.}
We conducted three crowd-sourcing experiments on 200 trainval images of PASCAL VOC 2007 to test the influence of using a qualification test and quality control. We report the quality of the bounding-boxes derived from extreme clicks in Tab.~\ref{tab:mturkInflQQ}.
%
Using a qualification test vastly improves annotation quality (from 75.4\% to 85.7\% mIoU).
The quality control brings a smaller further improvement to 87.1\% mIoU.

\begin{table}[t]
\vspace{-.1cm}
\centering
\small
\caption{\small Influence of the qualification test and quality control on the accuracy of extreme click annotations (on 200 images from PASCAL VOC 2007).}
\vspace{-.1cm}
\begin{tabular}{|c|c||c|c|} \hline
Qualification test & Quality control &  mIoU & IoU$>$0.7\\
\hline
 &  &  75.4 & 68.0\\
\checkmark &  & 85.7 & 91.0 \\
\checkmark & \checkmark & 87.1 & 92.5 \\
\hline
\end{tabular}
\vspace{-.5cm}
\label{tab:mturkInflQQ}
\end{table}

\subsection{Object detection performance}

To further validate our scheme for annotating bounding-boxes, we present experiments on training object class detectors from them, and compare to training from boxes manually drawn used the standard scheme \vitto{pascal-voc-g}, and to alternative ways to efficiently train detectors~\cite{bilen16cvpr,papadopoulos16cvpr}.

For PASCAL VOC 2007 we test the object detectors on the test set (4,952 images), while for PASCAL VOC 2012 we test them on the validation set (5,823 images). Below, in this subsection we discuss the results only on VOC 2007 as the same conclusions hold on for PASCAL VOC 2012. The complete mAP results for both datasets can be seen in Tab.~\ref{sec:resultsDet}. 

\mypar{Object detection model and evaluation.}
As object detector we use Fast R-CNN~\cite{girshick15iccv} with EdgeBoxes~\cite{dollar14eccv} as object proposals. We use both AlexNet~\cite{krizhevsky12nips} and VGG16~\cite{simonyan15iclr} as underlying CNN architectures.
%
We measure the performance of the trained object detector on the test set using mean average precision (mAP).

\mypar{PASCAL ground-truth bounding-boxes~\cite{pascal07:thomas}.}
Training object detectors from PASCAL ground-truth bounding-boxes results in 55.5\% mAP using AlexNet and 65.9\% mAP using the deeper VGG16 architecture.

\mypar{Extreme click annotations.}
The object detectors trained from bounding boxes derived from our extreme click annotation yield 56.0\% (AlexNet) and 66.1\% (VGG16) mAP. Interestingly, these detectors match the performance of those trained on the original, manually drawn ground-truth boxes. This confirms the quality of the boxes produced by our annotation scheme is as good as the original ground truth. Importantly, our scheme requires $5\times$ less annotation time.

\mypar{Weakly-supervised object localization~\cite{bilen16cvpr}.}
As a reference, we report here the mAP performance of Bilen et al.~\cite{bilen16cvpr}, a state-of-the-art WSOL technique. WSOL techniques are very cheap in terms of annotation time but their mAP performance (34.8\% with VGG16) is just over half of what we achieve with a detector trained on extreme clicks.

\mypar{Human verification scheme~\cite{papadopoulos16cvpr}.}

\dimpp{just mention mAP. 90\% of mAP}

\vitto{unconvincing! Focus on BBs produced at training time: from their paper you can claim a certain CorLoc @ IoU$>$0.5; we ROCK on that measure! Then as corroborating evidence you can state they reach only about 90\% of the mAP of training from gt bbs}

\mypar{Oracle best window proposals.}
\vitto{fuse with sec. 3.3}
We also train object detectors on the oracle best EdgeBox window proposal~\cite{dollar14eccv}. This yields 54.0\% mAP using AlexNet and 65.4\% mAP using VGG16. These mAPs can be seen as an upper-bound for any learning algorithm based on selecting object proposals. This includes most WSOL~\cite{bilen16cvpr,cinbis15pami,deselaers12ijcv,russakovsky12eccv,siva11iccv} and the human verification scheme~\cite{papadopoulos16cvpr}.
The object detectors trained on our extreme clicks go even slightly beyond this upper-bound ($+1\%$ mAP \vitto{pending result on VOC12}).



